Fast and Actionable Classification of HPC I/O Time Series

Input/output (I/O) is a major bottleneck for highperformance computing (HPC) performance. One of the challenges is the contention between jobs when sharing the parallel file system. However, tackling this issue depends on knowing the temporal behavior of jobs. In this paper, we propose a clusteringbased approach to characterize jobs' temporal I/O behavior. We propose SAGE, a lightweight method that cuts I/O traces into short windows and learns an alphabet from them. The trace then becomes a sequence of symbols, which we call ''genome'', and we use clustering to separate them into classes. We evaluate SAGE and its two-stage variant SAGE-2 on 819,771 real traces from 2 HPC systems. We compare them against other techniques from the state of the art on three metrics, including one we propose. Compared to K-shape, the best baseline available, SAGE-2 lowers the median intra-cluster metrics by 9.1% on average, and achieves this in 2 minutes of clustering time versus 3.8 hours, a 109x speedup. More importantly, clusters created by SAGE and SAGE-2 carry enough information to act on: we evaluate the use of the cluster centroids for I/O scheduling, and show that our approach can decrease I/O stretch by up to 24% compared to the state of the art (round-robin placement).

==> Makefile <==
MAIN    = main
RR      = $(MAIN)_research_report
LATEX   = pdflatex
BIBTEX  = bibtex
LFLAGS  = -halt-on-error

RRSRC   = '\def\researchreport{}\input{$(MAIN)}'

all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex ref.bib sections/*.tex
	$(LATEX) $(LFLAGS) $(MAIN)
	$(BIBTEX) $(MAIN)
	$(LATEX) $(LFLAGS) $(MAIN)
	$(LATEX) $(LFLAGS) $(MAIN)
	$(MAKE) clean-aux

# Order-only on the paper so the two builds never run at the same time under
# make -j (the comment package writes a shared comment.cut scratch file).
$(RR).pdf: $(MAIN).tex ref.bib | $(MAIN).pdf
	$(LATEX) $(LFLAGS) -jobname=$(RR) $(RRSRC)
	$(BIBTEX) $(RR)
	$(LATEX) $(LFLAGS) -jobname=$(RR) $(RRSRC)
	$(LATEX) $(LFLAGS) -jobname=$(RR) $(RRSRC)
	$(MAKE) clean-aux

clean-aux:
	for j in $(MAIN) $(RR); do \
	  rm -f $$j.aux $$j.bbl $$j.blg $$j.log $$j.out $$j.toc $$j.lof $$j.lot \
	        $$j.fls $$j.fdb_latexmk $$j.synctex.gz; \
	done
	rm -f comment.cut

clean: clean-aux
	rm -f $(MAIN).pdf $(RR).pdf

# The builds share the comment.cut scratch file, so never run them in parallel.
.NOTPARALLEL:

.PHONY: all clean clean-aux

